Bayesian Language Decision: Looking Back and Planning Ahead

System I decision models select among candidate actions directly, whereas System II models allocate additional inference-time computation to deliberative planning. Pairing the two lets a fast actor pursue long-horizon plans without invoking the planner at every step. Between planner calls, however, each decision must weigh what recent interactions reveal against where the plan points. We treat this trade-off as Bayesian inference over actions, with the past forming a prior and the planned future serving as evidence. Scoring this evidence directly would require knowing where each action leads. Under a simple factorization, Bayes' rule instead recasts it as how much the planned future raises or lowers each action's probability under the actor itself. We introduce Bayesian Language Decision (BLaDe), a training-free framework that queries one frozen actor under three contexts (the observation alone, with recent history, and with the planner's target) and combines the answers through a single weight $w$ that sets how far the plan may override the past. Across three System I models and four interactive benchmarks, BLaDe improves success over the actor alone in every actor-environment pair, raising average success from 14.76% to 40.38% at w=2 and cutting environment actions on ALFWorld household tasks by up to 52.5%, all without updating the actor.

==> figures/history_length_figure.tex <==
\begin{figure}[!htbp]
\centering
\IfFileExists{figures/history_length_babyai.pdf}{%
\includegraphics[width=0.76\linewidth]{figures/history_length_babyai.pdf}%
}{\input{figures/history_length_plot.tex}}
\caption{\textbf{Actor history length at fixed $w=2$.} d3 native task-success rates in an independent experiment on all 125 BabyAI cases at $\ell=0,4,8,12$ (500 completed episodes). Only the actor's history window changes; the planner always receives the four most recent interactions ($\ell_{\mathcal G}=4$) under the same fixed update schedule (Appendix~\ref{app:full-history-ablation}).}
\label{fig:history-length-babyai}
\end{figure}

